Hybrid Quantum Classical Graph Neural Networks for Particle Track Reconstruction

The Large Hadron Collider (LHC) at the European Organisation for Nuclear Research (CERN) will be upgraded to further increase the instantaneous rate of particle collisions (luminosity) and become the High Luminosity LHC (HL-LHC). This increase in luminosity will significantly increase the number of particles interacting with the detector. The interaction of particles with a detector is referred to as "hit". The HL-LHC will yield many more detector hits, which will pose a combinatorial challenge by using reconstruction algorithms to determine particle trajectories from those hits. This work explores the possibility of converting a novel Graph Neural Network model, that can optimally take into account the sparse nature of the tracking detector data and their complex geometry, to a Hybrid Quantum-Classical Graph Neural Network that benefits from using Variational Quantum layers. We show that this hybrid model can perform similar to the classical approach. Also, we explore Parametrized Quantum Circuits (PQC) with different expressibility and entangling capacities, and compare their training performance in order to quantify the expected benefits. These results can be used to build a future road map to further develop circuit based Hybrid Quantum-Classical Graph Neural Networks.

==> temp.tex <==
\begin{figure*}[!ht]
\centering
\begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[height=0.5\linewidth]{MPS.pdf}
    \caption{Matrix Product State (MPS) circuit. Adapted from~\cite{mps}.}
    \label{fig:MPS}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[height=0.5\linewidth]{TTN.pdf}
    \caption{Tree Tensor Network (TTN) circuit. Adapted from~\cite{ttn}.}
    \label{fig:TTN}
\end{subfigure}
\par\bigskip % force a bit of vertical whitespace
\begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[height=0.5\linewidth]{qc19.pdf}
    \caption{Circuit 19 in four qubits and single layer configuration. Adapted from~\cite{qc-assesment}.}
    \label{fig:c19}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.45\linewidth}
    \centering
    \includegraphics[height=0.5\linewidth]{qc10.pdf}
    \caption{Circuit 10 in four qubits and single layer configuration. Adapted from~\cite{qc-assesment}.}
    \label{fig:c10}
\end{subfigure}\\
\caption{Hierarchical (a, b) and layered (c, d) PQCs used in the HNN. (a) MPS applies two-qubit gates with a ladder-like architecture, (b) while TTN uses a tree-like architecture implement $R_Y$ and $CZ$ gates. MPS and TTN circuits measure only one qubit at the end. (c) Circuit 19 employs $R_X$, $R_Z$ and $CRX$ gates in a nearest neighbour fashion, (d) while Circuit 10 do this with $R_Y$ and $CZ$ gates. Circuit 10 and Circuit 19 can be extended to any number of layers by repating the circuit. Circuit 10 and Circuit 19 measure all qubits available.}
\label{fig:pqcs}
\end{figure*}


\begin{figure*}[!ht]
\begin{subfigure}[b]{.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{embedding_loss.pdf}
    \caption{Axis of angle embedding comparison.}
    \label{fig:embedding_comparison}
\end{subfigure}
\begin{subfigure}[b]{.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{layers_loss.pdf}
    \caption{Number of layers ($N_L$) comparison.}
    \label{fig:layer_comparison}
\end{subfigure}

\begin{subfigure}[b]{.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{iterations_loss.pdf}
    \caption{Number of iterations ($N_{I}$) comparison.}
    \label{fig:iteration_comparison}
\end{subfigure}
\begin{subfigure}[b]{.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{dim_loss.pdf}
    \caption{Hidden dimension size ($N_D=N_Q$) comparison.}
    \label{fig:dimension_comparison}
\end{subfigure}
\caption{Best validation loss comparison with respect to different parameters of the hybrid GNN model.  (a) The axis of angle embedding comparison considers the best loss obtained for different embedding axes by setting $N_D=N_Q=4$, $N_L=1$ and $N_I=3$. (b) The number of layers comparison considers the best loss for various numbers of layers ($N_L$) by setting $N_D=N_Q=4$ and $N_I=3$. (c) The number of iterations comparison considers the best loss for different numbers of iterations ($N_{I}$) by setting $N_D=N_Q=4$ and $N_L=1$. (d) The hidden dimension size comparison considers the loss for different hidden dimension sizes ($N_D$) by setting $N_Q=N_D$, $N_L=1$ and $N_I=3$. 5 instances of all models with different initial parameters are trained for 10 or 20 epochs depending on complexity for each setting, and the mean of best losses are presented. The error bars represent the $\pm$ standard deviation of the best losses of all 5 runs.}
\label{fig:comparisons}
\end{figure*}
